R2-D2: A Modular Baseline for Open-Domain Question Answering

This work presents a novel four-stage open-domain QA pipeline R2-D2 (Rank twice, reaD twice). The pipeline is composed of a retriever, passage reranker, extractive reader, generative reader and a mechanism that aggregates the final prediction from all system's components. We demonstrate its strength across three open-domain QA datasets: NaturalQuestions, TriviaQA and EfficientQA, surpassing state-of-the-art on the first two. Our analysis demonstrates that: (i) combining extractive and generative reader yields absolute improvements up to 5 exact match and it is at least twice as effective as the posterior averaging ensemble of the same models with different parameters, (ii) the extractive reader with fewer parameters can match the performance of the generative reader on extractive QA datasets.

==> figures/answer-reranking-v2.tex <==
\def\col{4.20cm}
\def\row{2.10cm}
\def\blockwidth{3.4cm}
\def\blockheight{1.0cm}
\def\arrowrate{0.3}

\newcommand\Textbox[2]{%
    \parbox[c][\dimexpr#1-7.7pt][c]{2.3cm}{\centering#2}}

\begin{tikzpicture}[->,line width=2pt,>=latex,node distance=\lvspace,
                    font=\footnotesize,
                    thick,
                    data/.style={line width=1pt,rectangle,draw, minimum width=\blockwidth, minimum height=2ex, align=center, rounded corners=0.1cm, fill=blue!20},
                    module/.style={
                        line width=1pt,
                        rectangle split, 
                        rectangle split parts=2,
                        rectangle split part fill={blue!30, gray!20},
                        draw,
                        minimum width=\blockwidth, 
                        align=center, 
                        rounded corners=0.1cm,
                    }
                ]

    \node[data, fill=cyan!30]  (RRp_o) at (1*\col,3*\row) {reranked passages \\ from passage reranker};
    \node[data, fill=green!30] (ER_o) at (0*\col,2*\row) {top-k answer spans \\ from extractive reader};
    \node[data, fill=blue!30] (R_o) at (0*\col,1.5*\row-0.15cm) {ranked passage scores \\ from retriever};
    \node[data, fill=cyan!30] (RR_o) at (0*\col,1*\row-0.3cm) {reranked passage scores \\ from passage reranker};
    \node[data, fill=yellow!30] (AR_o) at (0*\col,0*\row) {top generated answer \\ from abstractive reader};

    \node[module, rectangle split part fill={yellow!30, gray!30}]   at (1*\col,2*\row) (AR)    []                {\Textbox{\blockheight}{Abstractive reader}\nodepart{two}{reranked answer spans}};
    \node[module, rectangle split part fill={red!30, gray!30}]   at (1*\col,1*\row) (LF)                      {\Textbox{\blockheight}{score aggregation}\nodepart{two}{top span answer}};
    \node[module, rectangle split part fill={red!30, gray!30}]   at (1*\col,0*\row) (BD)    []                {\Textbox{\blockheight}{Binary decision}\nodepart{two}{top answer}};

    \draw[->,rounded corners] (RRp_o) to (AR);
    \draw[->,rounded corners] (ER_o) to (AR);
    \draw[->,rounded corners] (ER_o) to ($(ER_o.east)!0.6!(LF.west|-ER_o.east)$) to ($(LF.west-|ER_o.east)!0.6!(LF.west)+(0,0.3cm)$) to ($(LF.west)+(0,0.3cm)$);
    \draw[->,rounded corners] (R_o) to ($(R_o.east)!0.3!(LF.west|-R_o.east)$) to ($(LF.west-|ER_o.east)!0.3!(LF.west)$)  to (LF.west);
    \draw[->,rounded corners] (RR_o) to ($(LF.west)-(0,0.3cm)$);
    \draw[->,rounded corners] (AR) to (LF);
    \draw[->,rounded corners] (LF) to (BD);
    \draw[->,rounded corners] (AR_o) to (BD);
\end{tikzpicture}

==> figures/answer-reranking.tex <==
\def\col{4.20cm}
\def\row{2.10cm}
\def\blockwidth{3.3cm}
\begin{tikzpicture}[->,line width=2pt,>=latex,node distance=\lvspace,
                    font=\footnotesize,
                    thick,
                    module/.style={line width=1pt,rectangle,draw, minimum width=\blockwidth, minimum height=2ex, align=center, rounded corners=0.1cm, minimum height=1.0cm,fill=red!30},
                    data/.style={line width=1pt,rectangle,draw, minimum width=\blockwidth, minimum height=2ex, align=center, rounded corners=0.1cm, fill=blue!20},]

    \node[data, fill=green!30] (ER_o) at (0*\col,2*\row) {top-k answer spans \\ from extractive reader};
    \node[data, fill=blue!30] (R_o) at (0*\col,1.5*\row-0.15cm) {ranked passage scores \\ from retriever};
    \node[data, fill=red!30] (RR_o) at (0*\col,1*\row-0.3cm) {reranked passage scores \\ from passage reranker};
    \node[data, fill=yellow!30] (AR_o) at (0*\col,0*\row) {top generated answer \\ from abstractive reader};

    \node[module, fill=yellow!30]   at (1*\col,2*\row) (AR)    []                {Abstractive reader};
    \node[data]                        (ARR_o) [below=0cm of AR] {reranked answer spans};
    \node[module, fill=cyan!30]   at (1*\col,1*\row) (LF)                      {log-prob fusion};
    \node[data]                        (LF_o)  [below=0cm of LF] {top span answer};
    \node[module, fill=cyan!30]   at (1*\col,0*\row) (BD)    []                {Binary decision};
    \node[data]                        (BD_o)  [below=0cm of BD] {top answer};

    \draw[->,rounded corners] (ER_o) to (AR);
    \draw[->,rounded corners] (ER_o) to ($(ER_o.east)!0.6!(LF.west|-ER_o.east)$) to ($(LF.west-|ER_o.east)!0.6!(LF.west)+(0,0.3cm)$) to ($(LF.west)+(0,0.3cm)$);
    \draw[->,rounded corners] (R_o) to ($(R_o.east)!0.3!(LF.west|-R_o.east)$) to ($(LF.west-|ER_o.east)!0.3!(LF.west)$)  to (LF.west);
    \draw[->,rounded corners] (RR_o) to ($(LF.west)-(0,0.3cm)$);
    \draw[->,rounded corners] (ARR_o) to (LF);
    \draw[->,rounded corners] (LF_o) to (BD);
    \draw[->,rounded corners] (AR_o) to (BD);
\end{tikzpicture}

==> figures/pipeline-v2.tex <==
\def\col{2.00cm}
%\def\row{2.70cm}
\def\row{3.30cm}
\def\blockwidth{3.1cm}
\def\blockwidthlarge{7.1cm}
\def\blockheight{0.90cm}
\def\arrowrate{0.3}

\def\outputcolor{gray!20}
\def\examplecolor{white}

\newcommand\Textbox[2]{%
    \parbox[c][\dimexpr#1-7.7pt][c]{2.3cm}{\centering{#2}}}

\begin{tikzpicture}[->,line width=2pt,>=latex,node distance=\lvspace,
                    font=\footnotesize,
                    thick,
                    module/.style={
                        line width=1pt,
                        rectangle split, 
                        rectangle split parts=3,
                        rectangle split part fill={blue!30, gray!20, gray!10},
                        draw,
                        text width=\blockwidth, 
                        align=center, 
                        rounded corners=0.1cm,
                    }
                ]

    \node[module,rectangle split part fill={blue!30, \outputcolor, \examplecolor}, text width=\blockwidthlarge]   at (1*\col,3*\row) (R)  {\Textbox{\blockheight}{Retriever}\nodepart{two}{top-K passages}\nodepart[align=left]{three}{1. The Big Bang Theory is an American... \\ 2. Leonard Hofstadter, Ph.D., is a fictional... \\ 3. Sheldon was born in 1980...}};
    \node[cylinder, draw, ,thick,aspect=0.2,
        minimum height=0.8cm,minimum width=1.0cm,
        shape border rotate=90, align=center] at (-0.5*\col,3.255*\row) (datastorage) {index};

    \node[align=center] at (1*\col,3.65*\row) (question) {\Large When was Sheldon born?};

    \node[module,rectangle split part fill={cyan!40, \outputcolor, \examplecolor}, text width=\blockwidthlarge]   at (1*\col,2*\row) (RR) {\Textbox{\blockheight}{Passage re-ranker}           \nodepart{two}{top-K re-ranked passages}\nodepart[align=left]{three}{1. Leonard Hofstadter, Ph.D., is a fictional... \\ 2. Sheldon was born in 1980... \\ 3. The Big Bang Theory is an American...}};
    \node[module,rectangle split part fill={green!30, \outputcolor, \examplecolor}]  at (0*\col,1*\row) (ER) {\Textbox{\blockheight}{Extractive reader}          \nodepart{two}{top-M answer spans}\nodepart[align=left]{three}{1. American \\ 2. Ph.D. \\ 3. 1980}};
    \node[module,rectangle split part fill={yellow!40, \outputcolor, \examplecolor}] at (2*\col,1*\row+2.1ex) (AR) {\Textbox{\blockheight}{Abstractive reader}         \nodepart{two}{top generated answer}\nodepart[align=left]{three}{1. 1981}};
    \node[module,rectangle split part fill={yellow!40, \outputcolor, \examplecolor}]    at (0*\col,0*\row) (ARR)  {\Textbox{\blockheight}{Abstractive reader}\nodepart{two}{top-M re-ranked spans}\nodepart[align=left]{three}{1. Ph.D. \\ 2. 1980 \\ 3. American}};
    \node[module,rectangle split part fill={red!30, \outputcolor, \examplecolor},]    at (0*\col,-1*\row) (AGGR)  {\Textbox{\blockheight}{score aggregation}\nodepart{two}{top-M aggr. spans}\nodepart[align=left]{three}{1. 1980 \\ 2. American \\ 3. Ph.D.}};
    \node[module,rectangle split part fill={red!40, \outputcolor, \examplecolor}]    at (1*\col,-2*\row+2.1ex) (BD)  {\Textbox{\blockheight}{binary decision}\nodepart{two}{top answer}\nodepart[align=left]{three}{1. 1980}};
    
    %\draw[->,rounded corners] (datastorage.south) to (R.north-|datastorage.south);
    \draw[->,rounded corners] (question.south) to (R.north-|question.south);
    \draw[->,rounded corners] (R) to (RR);
    \draw[->,rounded corners] (RR) to ($(RR.south)!\arrowrate!(ER.north-|RR.south)$) to ($(ER.north|-RR.south)!\arrowrate!(ER.north)$) to (ER.north);
    \draw[->,rounded corners] (RR) to ($(RR.south)!\arrowrate!(AR.north-|RR.south)$) to ($(AR.north|-RR.south)!\arrowrate!(AR.north)$) to (AR.north);
    \draw[->,rounded corners] (ER) to (ARR);
    \draw[->,rounded corners] (AR) to ($(AR.south)!0.92!(BD.north-|AR.south)$) to ($(BD.north|-AR.south)!0.92!(BD.north)+(0.5cm,0)$) to ($(BD.north)+(0.5cm,0)$);
    \draw[->,rounded corners] (RR) to ($(RR.south|-ARR.east)$) to (ARR.east);
    \draw[->,rounded corners] (RR) to ($(RR.south|-AGGR.east)$) to (AGGR.east);
    \draw[->,rounded corners] (ARR) to (AGGR);

    \draw[->,rounded corners] (AGGR) to ($(AGGR.south)!\arrowrate!(BD.north-|AGGR.south)$) to ($(BD.north|-AGGR.south)!\arrowrate!(BD.north)-(0.5cm,0)$) to ($(BD.north)-(0.5cm,0)$);
    
    \draw[->,rounded corners] (R) to ($(R.south)!\arrowrate!(RR.north-|R.south)$) to ($(R.south)!\arrowrate!(RR.north-|R.south)-(4.22cm, 0)$) to ($(AGGR)-(2.22cm,0)$) to (AGGR.west);
    
    \draw[->,rounded corners] (ER) to ($(ER.south)!\arrowrate!(ARR.north-|ER.south)$) to ($(ER.south)!\arrowrate!(ARR.north-|ER.south)-(2.00cm, 0)$) to ($(AGGR)-(2.00cm,-0.3cm)$) to ($(AGGR.west)+(0, 0.3cm)$);
\end{tikzpicture}

==> figures/pipeline.tex <==
\def\col{1.80cm}
\def\row{2.10cm}
\def\blockwidth{3.0cm}
\def\blockheight{1.0cm}
\def\arrowrate{0.3}

\newcommand\Textbox[2]{%
    \parbox[c][\dimexpr#1-7.7pt][c]{2.3cm}{\centering#2}}

\begin{tikzpicture}[->,line width=2pt,>=latex,node distance=\lvspace,
                    font=\footnotesize,
                    thick,
                    module/.style={
                        line width=1pt,
                        rectangle split, 
                        rectangle split parts=2,
                        rectangle split part fill={blue!30, gray!20},
                        draw,
                        minimum width=\blockwidth, 
                        align=center, 
                        rounded corners=0.1cm,
                    }
                ]

    \node[module,rectangle split part fill={blue!30, gray!20}]   at (1*\col,3*\row) (R)  {\Textbox{\blockheight}{Retriever}\nodepart{two}{ranked passages}};
    \node[cylinder, draw, ,thick,aspect=0.2,
        minimum height=1.5cm,minimum width=2.0cm,
        shape border rotate=90, align=center] at (-0.8*\col,2.95*\row) (datastorage) {wiki\\dense index};

    \node[module,rectangle split part fill={cyan!40, gray!20}]   at (1*\col,2*\row) (RR) {\Textbox{\blockheight}{Passage reranker}           \nodepart{two}reranked passages};
    \node[module,rectangle split part fill={green!30, gray!20}]  at (0*\col,1*\row) (ER) {\Textbox{\blockheight}{Extractive reader}          \nodepart{two}top-k answer spans};
    \node[module,rectangle split part fill={yellow!40, gray!20}] at (2*\col,1*\row) (AR) {\Textbox{\blockheight}{Abstractive reader}         \nodepart{two}top generated answer};
    \node[module,rectangle split part fill={red!30, gray!20}]    at (1*\col,0*\row) (F)  {\Textbox{\blockheight}{Answer reranking\\\& fusion}\nodepart{two}top answer};
    
    \draw[->,rounded corners] (R) to (RR);
    \draw[->,rounded corners] (datastorage.east|-R.west) to (R.west);
    \draw[->,rounded corners] (RR) to ($(RR.south)!\arrowrate!(ER.north-|RR.south)$) to ($(ER.north|-RR.south)!\arrowrate!(ER.north)$) to (ER.north);
    \draw[->,rounded corners] (RR) to ($(RR.south)!\arrowrate!(AR.north-|RR.south)$) to ($(AR.north|-RR.south)!\arrowrate!(AR.north)$) to (AR.north);
    \draw[->,rounded corners] (ER) to ($(ER.south)!\arrowrate!(F.north-|ER.south)$) to ($(F.north|-ER.south)!\arrowrate!(F.north)-(0.75cm,0)$) to ($(F.north)-(0.75cm,0)$);
    \draw[->,rounded corners] (AR) to ($(AR.south)!\arrowrate!(F.north-|AR.south)$) to ($(F.north|-AR.south)!\arrowrate!(F.north)+(0.75cm,0)$) to ($(F.north)+(0.75cm,0)$);
    \draw[->,rounded corners] (RR) to (F);

    \draw[->,rounded corners] (R) to ($(R.south)!\arrowrate!(RR.north-|R.south)$) to ($(R.south)!\arrowrate!(RR.north-|R.south)-(4.00cm, 0)$) to ($(F)-(4.00cm,0)$) to (F.west);
\end{tikzpicture}

==> tables/ablation-study-3.tex <==
\begin{tabular}{cc|rrr|rrr|rrr|rrr}
\toprule
\multirow{2}{*}{\textbf{Readers}} & \multirow{2}{*}{\textbf{Fusion}} & \multicolumn{3}{c|}{\textbf{NQ-Open (dev)}}            & \multicolumn{3}{c|}{\textbf{NQ-Open (test)}}           & \multicolumn{3}{c|}{\textbf{TQ-Open (test)}}           & \multicolumn{3}{c}{\textbf{EfficientQA}}             \\
                                  &                                  & \multicolumn{1}{c}{ret.}     & \multicolumn{1}{c}{+rr}     & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{ret.}     & \multicolumn{1}{c}{+rr}     & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{ret.}     & \multicolumn{1}{c}{+rr}     & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{ret.}     & \multicolumn{1}{c}{+rr}     & \multicolumn{1}{c}{$\Delta$} \\ \midrule
ext                               & -                                & 48.12 & 48.38          & 0.26                          & 50.78 & 50.72          & -0.06                         & 65.01 & 65.46          & 0.45                          & 47.00 & 47.56          & 0.56                         \\
gen                               & -                                & 48.30 & 49.40          & 1.10                          & 49.92 & 50.69          & 0.77                          & 65.38 & {\ul 69.14}    & 3.76                          & 44.83 & 47.33          & 2.50                         \\
ext+gen                           & naive                            & 49.14 & 49.99          & 0.85                          & 51.88 & 52.44          & 0.56                          & 66.17 & 68.01          & 1.84                          & 47.06 & 49.11          & 2.05                         \\
ext+gen                           & aggr                             & 50.87 & 51.80          & 0.93                          & 54.13 & 54.90          & 0.77                          & 67.42 & 68.66          & 1.24                          & 50.44 & 52.00          & 1.56                         \\
ext+gen                           & aggr+bd                          & 51.18 & \textbf{52.07} & 0.89                          & 54.07 & \textbf{54.99} & 0.92                          & 67.37 & \textbf{69.94} & 2.57                          & 49.72 & \textbf{52.22} & 2.50                         \\ \bottomrule
\end{tabular}

==> tables/ablation-study-wo-nq-open-dev-and-trivia-dev.tex <==
\begin{tabular}{ccc|rrr|rrr|rrr}
\toprule
\textbf{Passage}   & \multirow{2}{*}{\textbf{Readers}} & \multirow{2}{*}{\textbf{Fusion}} & \multicolumn{3}{c|}{\textbf{NQ-Open}}                                              & \multicolumn{3}{c|}{\textbf{TriviaQA}}                                             & \multicolumn{3}{c}{\textbf{EfficientQA}}                                         \\
\textbf{reranking} &                                   &                                  & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c}{$\Delta$} \\ \midrule
-                  & ext                               & -                                & 48.64                    & 50.78                   & -2.14                         & 63.18                    & 65.01                   & -1.83                         & 44.50                    & 47.00                   & -2.50                        \\
-                  & gen                               & -                                & 48.39                    & 49.92                   & -1.53                         & 63.72                    & 65.38                   & -1.66                         & 43.50                    & 44.83                   & -1.33                        \\
-                  & ext+gen                           & naive                            & 50.00                    & 51.88                   & -1.88                         & 64.04                    & 66.17                   & -2.13                         & 45.61                    & 47.06                   & -1.45                        \\
-                  & ext+gen                           & aggr                             & 51.94                    & 54.13                   & -2.19                         & 65.41                    & 67.42                   & -2.01                         & 47.50                    & 50.44                   & -2.94                        \\
-                  & ext+gen                           & aggr+bd                          & 51.88                    & 54.07                   & -2.19                         & 65.69                    & 67.37                   & -1.68                         & 47.28                    & 49.72                   & -2.44                        \\ \midrule
\checkmark         & ext                               & -                                & 48.92                    & 50.72                   & -1.80                         & 63.51                    & 65.46                   & -1.95                         & 45.06                    & 47.56                   & -2.50                        \\
\checkmark         & gen                               & -                                & 48.31                    & 50.69                   & -2.38                         & {\ul 67.18}              & {\ul 69.14}             & -1.96                         & 45.22                    & 47.33                   & -2.11                        \\
\checkmark         & ext+gen                           & naive                            & 50.33                    & 52.44                   & -2.11                         & 66.02                    & 68.01                   & -1.99                         & 46.78                    & 49.11                   & -2.33                        \\
\checkmark         & ext+gen                           & aggr                             & 52.38                    & 54.90                   & -2.52                         & 66.86                    & 68.66                   & -1.80                         & \textbf{49.44}           & 52.00                   & -2.56                        \\
\checkmark         & ext+gen                           & aggr+bd                          & \textbf{52.58}           & \textbf{54.99}          & -2.41                         & \textbf{67.96}           & \textbf{69.94}          & -1.98                         & 49.22                    & \textbf{52.22}          & -3.00                        \\ \bottomrule
\end{tabular}

==> tables/ablation-study-wo-trivia-dev.tex <==
\begin{tabular}{ccc|cccc}
\toprule
\textbf{Passage}   & \multirow{2}{*}{\textbf{Readers}} & \multirow{2}{*}{\textbf{Fusion}} & \multicolumn{1}{c}{\textbf{NQ-Open}} & \multicolumn{1}{c}{\textbf{NQ-Open}} & \multicolumn{1}{c}{\textbf{TQ-Open}} & \multicolumn{1}{c}{\textbf{EfficientQA}} \\
\textbf{reranking} &                                   &                                  & \multicolumn{1}{c}{(dev)}            & \multicolumn{1}{c}{(test)}           & \multicolumn{1}{c}{(test)}            & \multicolumn{1}{c}{(test)}               \\ \midrule
-                  & ext                               & -                                & 48.12                                 & 50.78                                 & 65.01                                  & 47.00                                    \\
-                  & gen                               & -                                & 48.30                                 & 49.92                                 & 65.38                                  & 44.83                                    \\
-                  & ext+gen                           & naive                            & 49.14                                 & 51.88                                 & 66.17                                  & 47.06                                    \\
-                  & ext+gen                           & aggr                             & 50.87                                 & 54.13                                 & 67.42                                  & 50.44                                    \\
-                  & ext+gen                           & aggr+bd                          & 51.18                                 & 54.07                                 & 67.37                                  & 49.72                                    \\ \midrule
\checkmark         & ext                               & -                                & 48.38                                 & 50.72                                 & 65.46                                  & 47.56                                    \\
\checkmark         & gen                               & -                                & 49.40                                 & 50.69                                 & {\ul 69.14}                            & 47.33                                    \\
\checkmark         & ext+gen                           & naive                            & 49.99                                 & 52.44                                 & 68.01                                  & 49.11                                    \\
\checkmark         & ext+gen                           & aggr                             & 51.80                                 & 54.90                                 & 68.66                                  & 52.00                                    \\
\checkmark         & ext+gen                           & aggr+bd                          & \textbf{52.07}                        & \textbf{54.99}                        & \textbf{69.94}                         & \textbf{52.22}                           \\ \bottomrule
\end{tabular}

==> tables/ablation-study.tex <==
\begin{tabular}{ccc|rrr|rrr|rrr|rrr|rrr}
\toprule
\textbf{Passage}   & \multirow{2}{*}{\textbf{Readers}} & \multirow{2}{*}{\textbf{Fusion}} & \multicolumn{3}{c|}{\textbf{NQ-Open (dev)}}                                        & \multicolumn{3}{c|}{\textbf{NQ-Open (test)}}                                       & \multicolumn{3}{c|}{\textbf{TriviaQA (dev)}}                                       & \multicolumn{3}{c|}{\textbf{TriviaQA (test)}}                                      & \multicolumn{3}{c}{\textbf{EfficientQA}}                                         \\
\textbf{reranking} &                                   &                                  & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c|}{$\Delta$} & \multicolumn{1}{c}{1.7M} & \multicolumn{1}{c}{21M} & \multicolumn{1}{c}{$\Delta$} \\ \midrule
-                  & ext                               & -                                & 46.53                    & 48.12                   & -1.59                         & 48.64                    & 50.78                   & -2.14                         & 62.70                    & 64.75                   & -2.05                         & 63.18                    & 65.01                   & -1.83                         & 44.50                    & 47.00                   & -2.50                        \\
-                  & gen                               & -                                & 46.23                    & 48.30                   & -2.07                         & 48.39                    & 49.92                   & -1.53                         & 63.31                    & 65.21                   & -1.90                         & 63.72                    & 65.38                   & -1.66                         & 43.50                    & 44.83                   & -1.33                        \\
-                  & ext+gen                           & naive                            & 47.05                    & 49.14                   & -2.09                         & 50.00                    & 51.88                   & -1.88                         & 63.55                    & 65.16                   & -1.61                         & 64.04                    & 66.17                   & -2.13                         & 45.61                    & 47.06                   & -1.45                        \\
-                  & ext+gen                           & aggr                             & 49.05                    & 50.87                   & -1.82                         & 51.94                    & 54.13                   & -2.19                         & 65.11                    & 66.82                   & -1.71                         & 65.41                    & 67.42                   & -2.01                         & 47.50                    & 50.44                   & -2.94                        \\
-                  & ext+gen                           & aggr+bd                          & 49.35                    & 51.18                   & -1.83                         & 51.88                    & 54.07                   & -2.19                         & 65.68                    & 67.08                   & -1.40                         & 65.69                    & 67.37                   & -1.68                         & 47.28                    & 49.72                   & -2.44                        \\ \midrule
\checkmark         & ext                               & -                                & 46.64                    & 48.38                   & -1.74                         & 48.92                    & 50.72                   & -1.80                         & 62.91                    & 64.92                   & -2.01                         & 63.51                    & 65.46                   & -1.95                         & 45.06                    & 47.56                   & -2.50                        \\
\checkmark         & gen                               & -                                & 47.11                    & 49.40                   & -2.29                         & 48.31                    & 50.69                   & -2.38                         & {\ul 66.50}              & {\ul 68.67}             & -2.17                         & {\ul 67.18}              & {\ul 69.14}             & -1.96                         & 45.22                    & 47.33                   & -2.11                        \\
\checkmark         & ext+gen                           & naive                            & 47.78                    & 49.99                   & -2.21                         & 50.33                    & 52.44                   & -2.11                         & 65.29                    & 67.43                   & -2.14                         & 66.02                    & 68.01                   & -1.99                         & 46.78                    & 49.11                   & -2.33                        \\
\checkmark         & ext+gen                           & aggr                             & 49.89                    & 51.80                   & -1.91                         & 52.38                    & 54.90                   & -2.52                         & 66.00                    & 68.12                   & -2.12                         & 66.86                    & 68.66                   & -1.80                         & \textbf{49.44}           & 52.00                   & -2.56                        \\
\checkmark         & ext+gen                           & aggr+bd                          & \textbf{50.25}           & \textbf{52.07}          & -1.82                         & \textbf{52.58}           & \textbf{54.99}          & -2.41                         & \textbf{67.41}           & \textbf{69.61}          & -2.20                         & \textbf{67.96}           & \textbf{69.94}          & -1.98                         & 49.22                    & \textbf{52.22}          & -3.00                        \\ \bottomrule
\end{tabular}

==> tables/dataset_statistics.tex <==
\def\tablepad{1ex}
\begin{tabular}{l r r r}
\toprule
    \multicolumn{1}{c}{\bf Dataset} & \multicolumn{1}{c}{\bf Train} & \multicolumn{1}{c}{\bf Dev} &     \multicolumn{1}{c}{\bf Test}  \\
    \midrule
    NQ-Open    & 79,168 & 8,757 & 3,610 \\
    \hspace{\tablepad} 
     - filt. reranker    & 71,238 & - & - \\
    \hspace{\tablepad}  
     - filt. ext. reader   & 61,755 & - & - \\
    \hspace{\tablepad} 
     - w/ golden passage  & 58,876 & 6,515  & - \\
    TQ-Open    & 78,785 & 8,837 & 11,313 \\
    \hspace{\tablepad} 
     - filt. reranker    & 69,346 & - & - \\
    \hspace{\tablepad} 
     - filt. ext. reader   & 62,332 & - & - \\
    \hspace{\tablepad} 
     - w/ golden passage    & 60,413 & 6,760 & - \\
    EfficientQA & -      & -       & 1,800 \\
    \midrule
    NQ-Golden       & \multicolumn{1}{c}{176,628} & 4,332  & 8,698 \\
    TQ-Golden       & \multicolumn{1}{c}{181,239} & 4,516  & 9,004 \\
\bottomrule
\end{tabular}

==> tables/fusion-analysis_binary-decision_efficientqa.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 48.33 & 50.06 & 49.39 & 49.67          \\
$\{g\}$   & 48.94 & 49.50 & 50.06 & 49.72          \\
$\{e,g\}$ & 50.78 & 51.83 & 50.94 & \textbf{52.22} \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_binary-decision_nq-open-dev.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 50.65 & 51.24          & 51.01 & 51.17 \\
$\{g\}$   & 50.36 & 50.91          & 50.68 & 50.90 \\
$\{e,g\}$ & 52.24 & \textbf{52.29} & 52.27 & 52.07 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_binary-decision_nq-open-test.tex <==
\begin{tabular}{cccccc}
\toprule
& $\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\small NQ-open}} & $\{e\}$   & 52.85 & 53.30          & 53.10 & 52.94 \\
                                                          & $\{g\}$   & 52.44 & 52.77          & 53.21 & 53.07 \\
                                                          & $\{e,g\}$ & 54.35 & \textbf{55.10} & 54.46 & 54.99 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_binary-decision_tq-open-dev.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 69.03 & 69.03 & 69.01 & 68.99 \\
$\{g\}$   & 69.54 & 69.46 & 69.62 & 69.70 \\
$\{e,g\}$ & 69.77 & \textbf{69.79} & 69.67 & 69.61 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_binary-decision_tq-open-test.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 69.34 & 69.28 & 69.23 & 69.26 \\
$\{g\}$   & 69.76 & 69.71 & 69.65 & 69.77 \\
$\{e,g\}$ & 69.80 & 69.89 & 69.88 & \textbf{69.94} \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_score-aggr_efficientqa.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 47.56 & 48.33 & 48.89 & 48.72          \\
$\{g\}$   & 49.11 & 49.56 & 50.22 & 50.11          \\
$\{e,g\}$ & 50.78 & 51.67 & 50.89 & \textbf{52.00} \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_score-aggr_nq-open-dev.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 48.38 & 48.94 & 48.85 & 49.14 \\
$\{g\}$   & 49.99 & 50.49 & 50.35 & 50.47 \\
$\{e,g\}$ & 51.79 & \textbf{51.97} & 51.82 & 51.80 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_score-aggr_nq-open-test.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 50.72 & 51.41          & 51.55 & 51.69 \\
$\{g\}$   & 52.44 & 52.88          & 53.35 & 53.19 \\
$\{e,g\}$ & 54.63 & \textbf{55.10} & 54.82 & 54.90 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_score-aggr_tq-open-dev.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 65.07 & 65.21 & 65.16 & 65.24 \\
$\{g\}$   & 67.68 & 67.72 & 67.73 & 67.76 \\
$\{e,g\}$ & 68.13 & \textbf{68.19} & 68.17 & 68.12 \\ \bottomrule
\end{tabular}

==> tables/fusion-analysis_score-aggr_tq-open-test.tex <==
\begin{tabular}{crrrr}
\toprule
$\boldsymbol{P}_*$ & \multicolumn{1}{c}{$\emptyset$} & \multicolumn{1}{c}{$\{r\}$} & \multicolumn{1}{c}{$\{rr\}$} & \multicolumn{1}{c}{$\{r,rr\}$} \\ \midrule
$\{e\}$   & 65.54 & 65.64 & 65.60 & 65.61 \\
$\{g\}$   & 68.25 & 68.17 & 68.21 & 68.26 \\
$\{e,g\}$ & 68.45 & 68.57 & \textbf{68.66} & \textbf{68.66} \\ \bottomrule
\end{tabular}

==> tables/joint-fusion-analysis.tex <==
\begin{tabular}{@{}crrrr@{}}
\toprule
\multirow{2}{*}{\textbf{$P_*$}} & \multicolumn{2}{c}{\textbf{NQ-open}}               & \multicolumn{2}{c}{\textbf{TriviaQA}}              \\
                                & \multicolumn{1}{c}{aggr} & \multicolumn{1}{c}{+bd} & \multicolumn{1}{c}{aggr} & \multicolumn{1}{c}{+bd} \\ \midrule
$\{e\}$                         & 50.72                    & 52.85                   &                          &                         \\
$\{e,r\}$                       &                          &                         &                          &                         \\
$\{e,rr\}$                      &                          &                         &                          &                         \\
$\{e,r,rr\}$                    &                          &                         &                          &                         \\
$\{g\}$                         &                          &                         &                          &                         \\
$\{g,r\}$                       &                          &                         &                          &                         \\
$\{g,rr\}$                      &                          &                         &                          &                         \\
$\{g,r,rr\}$                    &                          &                         &                          &                         \\
$\{e,g\}$                       &                          &                         &                          &                         \\
$\{e,g,r\}$                     & 55.10                    & 55.10                   &                          &                         \\
$\{e,g,rr\}$                    &                          &                         &                          &                         \\
$\{e,g,r,rr\}$                  & 54.90                    & 54.90                   &                          &                         \\ \bottomrule
\end{tabular}
